Quantum Field Theories, Topological Materials, and Topological Quantum Computing

A quantum computer can perform exponentially faster than its classical counterpart. It works on the principle of superposition. But due to the decoherence effect, the superposition of a quantum state gets destroyed by the interaction with the environment. It is a real challenge to completely isolate a quantum system to make it free of decoherence. This problem can be circumvented by the use of topological quantum phases of matter. These phases have quasiparticles excitations called anyons. The anyons are charge-flux composites and show exotic fractional statistics. When the order of exchange matters, then the anyons are called non-Abelian anyons. Majorana fermions in topological superconductors and quasiparticles in some quantum Hall states are non-Abelian anyons. Such topological phases of matter have a ground state degeneracy. The fusion of two or more non-Abelian anyons can result in a superposition of several anyons. The topological quantum gates are implemented by braiding and fusion of the non-Abelian anyons. The fault-tolerance is achieved through the topological degrees of freedom of anyons. Such degrees of freedom are non-local, hence inaccessible to the local perturbations. Ternary logic gates are more compact than their binary counterparts and naturally arise in a type of anyonic model called the metaplectic anyons. The mathematical model, for the fusion and braiding matrices of metaplectic anyons, is the quantum deformation of the recoupling theory. In this dissertation, we gave comprehensive background of topological quantum computation. Topology and knot theory, geometric phases, topological materials, topological quantum field theories, recoupling theory, and category theory are discussed. We proposed that the existing quantum ternary arithmetic gates can be realized by braiding and topological charge measurement of the metaplectic anyons.

==> 0_TitlePage.tex <==
\begin{titlepage}
	\title{\textbf{Quantum Field Theories, Topological Materials, and Topological Quantum Computation}\\
		\vspace{7mm}
		by\\
		Muhammad Ilyas\\
		\vspace{8mm}
	\large	A dissertation submitted in partial fulfillment of the requirements for the degree of \\
		\vspace{5mm}
		Doctor of Philosophy\\
		in\\
		Applied Physics\\		
		\vspace{8mm}
		Dissertation Committee:\\
		Marek Perkowski, Chair\\
		Jack Straton, Co-Chair\\
		Steven Bleiler\\
		Peter Leung\\
		Aslam Khalil\\
		\vspace{4mm}
		\centering
		\includegraphics[scale=0.4]{PSULogo}\\
		\vspace{5mm}
		{\Large Portland State University}}
	\date{2021}
\end{titlepage}
